Local Convergence of Adaptive Methods for Nonlinear Partial Differential Equations

In this article we develop convergence theory for a general class of adaptive approximation algorithms for abstract nonlinear operator equations on Banach spaces, and use the theory to obtain convergence results for practical adaptive finite element methods (AFEM) applied to several classes of nonlinear elliptic equations. In the first part of the paper, we develop a weak-* convergence framework for nonlinear operators, whose Gateaux derivatives are locally Lipschitz and satisfy a local inf-sup condition. The framework can be viewed as extending the recent convergence results for linear problems of Morin, Siebert and Veeser to a general nonlinear setting. We formulate an abstract adaptive approximation algorithm for nonlinear operator equations in Banach spaces with local structure. The weak-* convergence framework is then applied to this class of abstract locally adaptive algorithms, giving a general convergence result. The convergence result is then applied to a standard AFEM algorithm in the case of several semilinear and quasi-linear scalar elliptic equations and elliptic systems, including: a semilinear problem with subcritical nonlinearity, the steady Navier-Stokes equations, and a quasilinear problem with nonlinear diffusion. This yields several new AFEM convergence results for these nonlinear problems. In the second part of the paper we develop a second abstract convergence framework based on strong contraction, extending the recent contraction results for linear problems of Cascon, Kreuzer, Nochetto, and Siebert and of Mekchay and Nochetto to abstract nonlinear problems. The contraction result is then applied to a standard AFEM algorithm for semilinear problems with sub- and super-critical nonlinearities and for the Hamiltonian constraint in general relativity.

==> app.tex <==
\appendix

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{General Discussion Notes}

Summary of the discussion on 11/25/08.

\begin{itemize}
\item 
It may be a good idea to include the $p$-Laplacian problem as an example.
Then there is an issue of the continuous and uniform discrete inf-sup conditions.
Perhaps these can be tackled by monotonicity arguments.
\item 
Related to the above point, if the equation $F(u)=0$ can be considered as a minimization problem for some (strictly) convex functional,
or more generally, if we consider a minimization problem for such a functional which is not necessarily differentiable,
then it may be possible to take a completely different route that gives a very general proof by fully exploiting monotonicity.
Moreover,we might be able to obtain a linear convergence result in this case,
by relying on the equivalence between the energy- and the error reductions.
This will generalize quasi-orthogonality arguments since linear elliptic operators correspond to quadratic energies.
\item
The arguments in this paper can be easily modified to include the case $F:U\subset X\to Y^*$,
i.e., the case where the map $F$ is defined only on a subset of $X$.
Then we would need to guarantee that all the discrete solutions are in this subset, 
which can be done, e.g., in the case $U=H^1\cap\{u\in L^\infty:\alpha\leqs u\leqs\beta\;a.e.\}$, by using discrete maximum principles and so imposing various conditions on the mesh.
\item
Related to the above point, mesh conditions may be avoidable if we consider the problem in spaces such as
$H^1\cap L^q$, and contract the error in this space.
If one needs the convergence only in $H^1$-norm, it suffices to control the $L^q$ part of the error,
rather than reducing it.
\end{itemize}

There was a discussion as to what is the dual of $H^1\cap L^q$.
This is answered essentially in Section 2.7 of the book by Bergh and L\"ofstr\"om, which we summarize below.

Let $A$ and $B$ be normed vector spaces, both are subspaces of a Hausdorff topological vector space $U$.
Then we define their {\em intersection} $A\cap B$ and {\em sum} $A+B$ as normed vector spaces with norms
$$
\|u\|_{A\cap B}=\max\{\|u\|_A,\|u\|_B\},\qquad
\|u\|_{A+B}=\inf_{u=a+b}\{\|a\|_A+\|b\|_B\},
$$
respectively.

Recall that the {\em direct sum} $A\oplus B$ is the normed vector space 
consisting of the ordered pairs $(a,b)$, $a\in A$, $b\in B$,
equipped with the norm
$\|(a,b)\|_{A\oplus B}=\max\{\|a\|_A,\|b\|_B\}$.
Then the subspace
$$
E=\{(a,b)\in A\oplus B:a=b\},
$$
is isometrically isomorphic to $A\cap B$.
Moreover, one can show that $(A\oplus B)/E$, equipped with the quotient norm, is
isometrically isomorphic to $A+B$.

Now suppose that $A$ and $B$ are Banach spaces.
Then it is easy to see that their intersection, sum, and direct sum are also Banach spaces.

\begin{theorem}
If $A\cap B$ is dense in both $A$ and $B$,
then $(A\cap B)'=A'+B'$ and $(A+B)'=A'\cap B'$.
\end{theorem}

\begin{proof}
We will only prove the first assertion.
Let $f\in A'+B'$ and $f=g+h$  with $g\in A'$ and $h\in B'$.
Then for $u\in A\cap B$ we have
$$
\ang{f,u}
\leqs 
|\ang{g,u}|+|\ang{h,u}|
\leqs
\left(\|g\|_{A'}+\|h\|_{B'}\right)\max\{\|u\|_A,\|u\|_B\},
$$
so $f\in(A\cap B)'$ and $\|f\|_{(A\cap B)'}\leqs \|f\|_{A'+B'}$.

Conversely, let $f\in (A\cap B)'$, i.e., $f(u)\leqs \|f\|_{(A\cap B)'}\|u\|_{A\cap B}$ for $u\in A\cap B$.
Let $\varphi$ be a linear functional on $E$ defined as
$\varphi:(a,b)\mapsto \frac12f(a+b)$.
This functional is bounded on $E$:
\begin{equation*}
\begin{split}
\varphi(a,b)
&\leqs
\textstyle\frac12\|f\|_{(A\cap B)'}(\|a\|_{A\cap B}+\|b\|_{A\cap B})
\\
&=
\|f\|_{(A\cap B)'}\|a\|_{A\cap B}
\\
&=
\|f\|_{(A\cap B)'}\max\{\|a\|_{A},\|a\|_{B}\}
\\
&=
\|f\|_{(A\cap B)'}\max\{\|a\|_{A},\|b\|_{B}\}
\\
&=
\|f\|_{(A\cap B)'}\|(a,b)\|_{A\oplus B}.
\end{split}
\end{equation*}
Now by the Hahn-Banach theorem, there exists an extension $\psi\in(A\oplus B)'$ of $\varphi$
with the same norm as that of $\varphi$, i.e.,
$\psi(a,b)=\varphi(a,b)$ for $(a,b)\in E$, and $\|\psi\|_{(A\oplus B)'}\leqs \|f\|_{(A\cap B)'}$.
Since $(A\oplus B)'=A'\oplus B'$, this means that there exists a pair $(g,h)\in A'\oplus B'$ such that
$$
\varphi(a,b)=g(a)+h(b),\quad (a,b)\in E,
\qquad
\textrm{and}
\qquad
\max\{\|g\|_{A'},\|h\|_{B'}\}\leqs \|f\|_{(A\cap B)'}.
$$
Thus, taking $a=b=u\in A\cap B$, we have
$$
f(u)=\varphi(u,u)=g(u)+h(u),
\qquad u\in A\cap B,
$$
and so by the density assumption, $f=g+h$.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Some thoughts on quasi-orthogonality}

The (quasi-)orthogonality is an essential ingredient in proving the linear convergence of adaptive algorithms for linear elliptic equations (cf.~\cite{Morin.P;Nochetto.R;Siebert.K2002, Mekchay.K;Nochetto.R2005,Cascon.J;Kreuzer.C;Nochetto.R;Siebert.K2007}).
In the following section, we list some rough ideas on understanding the orthogonality, and possibly generalize these ideas.

We consider the following general semi-linear elliptic problem and it's finite element approximation:
\begin{eqnarray*}
(\nabla u, \nabla v) &=& (f(u), v),\quad \forall v\in H_0^1(\Omega)\\
(\nabla u_h, \nabla v) &=& (f(u_h), v),\quad \forall v\in V_h\subset H_0^1(\Omega)
\end{eqnarray*}
It is straightforward to get the following identity:
\begin{equation}\label{eq:orthogonality}
|u-u_h|_{1}^2 = |u-v_h|_{1}^2 - |u_h - v_h|_{1}^2 + 2(f(u)-f(u_h), v_h - u_h).
\end{equation}
The quasi-orthogonality relation is then characterized by the cross term
$$(f(u)-f(u_h), v_h - u_h).$$

In adaptive algorithm setting, we usually have $v_h = u_H$ where $u_H \in V_H \subset V_h.$
In order to get certain reduction, we want to have some control of the upper bound of this cross term.
Namely, we want
$$(f(u)-f(u_h), u_H - u_h)\leqs \epsilon(|u-u_h|_1) +p(|u_H - u_h|_1),$$
where $\epsilon$ should be small.

As a naive example, let $f:=f(x)$ be independent of $u.$ Then the cross term disappear, and the above relation is the standard Galerkin orthogonality.

Take $f(x, u) = g(x) - {\bf b} \cdot \nabla u$ as another example, then we have the following quasi-orthogonality (cf.~\cite{Mekchay.K;Nochetto.R2005}):
$$(f(u)-f(u_h), v_h - u_h)\leqs C\delta h^s\|u-u_h|_{1}^2 + \frac{C(b)}{\delta} |v_h - u_h|_1^2.$$

We consider the following general semi-linear elliptic problem and it's finite element approximation:
\begin{eqnarray*}
(\nabla u, \nabla v) &=& (f(u), v),\quad \forall v\in H_0^1(\Omega)\\
(\nabla u_h, \nabla v) &=& (f(u_h), v),\quad \forall v\in V_h\subset H_0^1(\Omega)
\end{eqnarray*}
It is straightforward to get the following identity:
\begin{equation}\label{eq:orthogonality2}
|u-u_h|_{1}^2 = |u-v_h|_{1}^2 - |u_h - v_h|_{1}^2 + 2(f(u)-f(u_h), v_h - u_h).
\end{equation}
The quasi-orthogonality relation is then characterized by the cross term
$$(f(u)-f(u_h), v_h - u_h).$$

In adaptive algorithm setting, we usually have $v_h = u_H$ where $u_H \in V_H \subset V_h.$
In order to get certain reduction, we want to have some control of the upper bound of this cross term.
Namely, we want
$$(f(u)-f(u_h), u_H - u_h)\leqs \epsilon(|u-u_h|_1) +p(|u_H - u_h|_1),$$
where $\epsilon$ should be small.

As a naive example, let $f:=f(x)$ be independent of $u.$ Then the cross term disappear, and the above relation is the standard Galerkin orthogonality.

Take $f(x, u) = g(x) - {\bf b} \cdot \nabla u$ as another example, then we have the following quasi-orthogonality (cf.~\cite{Mekchay.K;Nochetto.R2005}):
$$(f(u)-f(u_h), v_h - u_h)\leqs C\delta h^s\|u-u_h|_{1}^2 + \frac{C(b)}{\delta} |v_h - u_h|_1^2.$$

For general semi-linear problems, to get the quasi-orthogonality we need some inequality like (cf.~\cite{HoTs07b,Chen.L;Holst.M;Xu.J2007})
$$\|f(u) - f(v)\| \leqs C \|u-v\|.$$

From hypercircle point of view, when $f$ is independent of $u,$ then 
$\nabla u,$ $\nabla u_h$ and $\nabla v_h$ lie on the hypercircle with the center $\frac{\nabla u + \nabla v_h}{2}$ and diameter $|u - v_h|_1.$
In general case, in order to have good control of the error, we want $u_h$ to lie inside (or not too far away from) the hypercircle.
Ideally, this is equivalent to the condition 
$$(f(u) - f(u_h), v_h - u_h) \leqs 0.$$


Questions:
\begin{enumerate}
\item Can we generalize the quasi-orthogonality idea to more general class problem? For example, the bilinear form $b(\cdot, \cdot): V\times W \to R,$ which satisfies the inf-sup conditions.
\item What is appropriate concept for Stokes problem?
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Some discussion on eigenvalue problem}

In this section, we discuss a little bit about the main idea of adaptive finite element method for the following eigenvalue problem:
\begin{equation}\label{eq:eigenvalue}
\left\{ \begin{array}{rlll}
-\div (A \nabla u) + b u &= & \lambda u & \mbox{in } \Omega,\\
u &=& 0 & \mbox{on } \partial \Omega.
\end{array}\right.
\end{equation}

So far, there are several approaches for the a posteriori error estimate for the finite element approximation of equation \eqref{eq:eigenvalue}.
In~\cite{Verfurth.R1994}, the eigenvalue problem was treated as a bifurcation problem, or as a nonlinear equation by adding the constraint $\|u\|_{0,\Omega}=1.$

Another approach, due to~\cite{Dai.X;Xu.J;Zhou.A2008}, is to treat the equation \eqref{eq:eigenvalue} as a perturbation of linear equations.
More precisely, we want to solve the eigenvalue problem: Find $(\lambda, u) \in \R \times H_0^1(\Omega)$ such that  
\begin{equation}\label{eq:eig-weak}
a(u,v) := (A u, v) + (bu, v) = (\lambda u, v),\quad \forall v\in H_0^1(\Omega).
\end{equation}
By the finite element approximation, we find $(\lambda_h, u_h) \in \R \times V_h$ such that  
\begin{equation}\label{eq:eig-fem}
a(u_h, v_h) = (\lambda_h u_h, v_h),\quad \forall v_h\in V_h.
\end{equation}
The Galerkin solution $u_h\in V_h$ of equation \eqref{eq:eig-fem} can be viewed as the solution of the following (continuous) equation with the right hand side $\lambda_h u_h$: Find $w\in H_0^1(\Omega)$ such that  
\begin{equation}\label{eq:eig-perturb}
a(w,v)  = (\lambda_h u_h, v),\quad \forall v\in H_0^1(\Omega).
\end{equation}
By triangle inequality, we have
$$\|u-u_h\|_{a, \Omega} \leqs \|u-w\|_{a, \Omega} + \|w - u_h\|_{a,\Omega}.$$
It was proved in~\cite[Theorem 3.1]{Dai.X;Xu.J;Zhou.A2008} that
$$\|u- w\|_{a,\Omega} \leqs C r(h) \|u - u_h\|_{a,\Omega},$$
where $r(h):= C(h, \Omega) + \|u-u_h\|_{a,\Omega}$ and $C(h, \Omega)\to 0$ as $h\to 0,$  depends on the regularity and the shape of domain.
That is, up to a higher order term, $\|u-u_h\|_{a,\Omega}$ is bounded by $\|w-u_h\|_{a, \Omega}.$

Notice problem \eqref{eq:eig-perturb} is a usual elliptic boundary value problem, we have the standard a posteriori error analysis for $\|w-u_h\|_{a,\Omega}.$ Combining with the above discussion, we obtain the a posteriori error estimates for $\|u-u_h\|_{a,\Omega}.$ The convergence and the complexity of AFEM also follows by this relation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Some Notes Related to Newton's Method}

We consider the contraction of residual of type 
$$ \|F(u_{k+1})\| \leqs \|F(u_k)\|.$$
For this purpose, we start with the Taylor expansion:
\begin{equation}
\label{eqn:taylor}
F(u_{k+1}) = F(u_k) + F'(u_k)(u_{k+1}) - F(u_k)) + \int_{0}^1 \left( F'(u_k + s (u_{k+1} - u_k)) - F'(u_k)\right) (u_{k+1} - u_k) ds.
\end{equation}

Then we have 
$$ \|F(u_{k+1})\| = \|F(u_k)\|\left[  \sup_{v\in Y, \|v\|_Y =1} \langle A_k + B_k, v \rangle  \right],$$
where 
\begin{eqnarray*}
A_k &=& \|F(u_k)\|^{-1}(F'(u_k) (u_{k+1} - u_k) + F(u_k)),\\
B_k &=& \|F(u_k)\|^{-1}\int_{0}^1 \left( F'(u_k + s (u_{k+1} - u_k)) - F'(u_k)\right) (u_{k+1} - u_k) ds.
\end{eqnarray*}
Therefore, we have 
$$ \|F(u_{k+1})\| \leqs (\alpha_k + \beta_k) \|F(u_k)\|, $$
where $\alpha_k = \|A_k\|$ and $\beta_k = \|B_k\|.$
With the Lipschitz continuous assumption on $F'(\cdot),$ we may choose the ball sufficiently small such that $\beta_k$ is as small as we wish.
Therefore, we only need to control $\alpha_k.$

Let $\widetilde{u} \in X$ satisfies
\begin{equation}
\label{eqn:newton}
\langle F'(u_k) (\widetilde{u} - u_k), v\rangle + \langle F(u_k), v \rangle=0, \quad \forall v\in Y.
\end{equation}
That is, $\widetilde{u}$ is the EXACT solution of the Newton equation:
$$F'(u_k) (\widetilde{u} - u_k) + F(u_k) =0.$$
Thus we have the following
$$
A_k = \|F(u_k)\|^{-1}(F'(u_k) (u_{k+1} - \tilde{u}).
$$
Therefore $\alpha_k$ measures the difference of the finite element $u_{k+1}$ from the exact Newton solution $\tilde{u}.$

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Contraction based on Newton's Method}

Consider now the following problem:
\begin{equation}
\mathrm{Find}~u \in X ~\mathrm{such~that}~ J(u) \leqs J(v), 
  \quad \forall v \in X,
\end{equation}
where $J:X \rightarrow \mathbb{R}$.
We have then the associated subspace approximation problem:
\begin{equation}
\mathrm{Find}~u_h \in X_h \subset X ~\mathrm{such~that}~ J(u_h) \leqs J(v_h), 
  \quad \forall v_h \in X_h \subset X.
\end{equation}
We wish to develop conditions on $J$ and on the subspaces 
$X_h \subset X$ and $X_H \subset X$ that will ensure a contraction
of the form
\begin{equation}
E_h \leqs \gamma E_h, \quad 0 \leqs \gamma < 1,
\end{equation}
where $E_h = J(u_h) - J(u)$ and $E_H = J(u_H) - J(u)$,
with $u_h \in X_h$ and $u_H \in X_H.$
The natural case is $X_H \subseteq X_h$, but more generally
we might only have $\mathrm{dim}(X_H) \leqs \mathrm{dim}(X_h)$.

Assume that $J$ is sufficient smooth so that 
the Taylor formula holds (cf.~\cite{Zeid91c})
\begin{equation}
\begin{split}
J(u_h) &= J(u_H + [u_h - u_H]) \\
       &= J(u_H) + \langle \tilde{J}'(u_h,u_H),u_h-u_H\rangle,
\end{split}
\end{equation}
where the linear functional $\tilde{J}'$ representing the
Taylor remainder has the form
\begin{equation}
\langle \tilde{J}'(u_h,u_H),u_h-u_H \rangle
    = \langle \int_0^1 J'(tu_h + [1-t]u_H) dt, u_h-u_H \rangle.
\end{equation}

We now need to recall the notion of a descent direction.
\begin{definition}
Let $J:X \rightarrow \mathbb{R}$ be Gateaux differentiable at $u \in X$
in the direction $v \in X$.
We say $v$ is an $\alpha$-descent direction of $J$ at $u$ if
\begin{equation}
\langle J'(u), v \rangle \leqs -\alpha \|v\|^2 < 0, \quad \alpha > 0.
\end{equation}
\end{definition}
We now need the following lemma.
\mnote{
The idea was to use sufficient descent on $J$ at $u$ to get
a sufficient descent-type condition on the Taylor remainder; to do
this we would need a Lemma like the following one.
This is not complete, but you get the idea. -mjh
}
\begin{lemma}
Let $J:X \rightarrow \mathbb{R}$ be $C^1$ in a ball around the
minimizer $u \in X$ which contains $v$ and $w$.
Let $w-v$ be an $\alpha$-descent direction of $J$ at $u$.
Then
\begin{equation}
\langle \tilde{J}'(v,w), v-w \rangle \leqs -\bar{\alpha} [J(w) - J(u)],
   \quad \bar{\alpha} \in (0,1).
\end{equation}
\end{lemma}
\begin{proof}
...
\end{proof}


We then have
\begin{theorem}
Let $J:X \rightarrow \mathbb{R}$ be $C^1$ in a ball around the
minimizer $u \in X$, which contains both $u_h$ and $u_H$.
If $J$ has sufficient descent at $u$ in the direction $v=u_h - u_H$,
then we have the contraction:
\begin{equation}
E_h \leqs \gamma E_H, \quad \gamma = [1 - \alpha] \in [0,1).
\end{equation}
\end{theorem}open mm.
\begin{proof}
We start with
\begin{equation}
\begin{split}
E_h &= J(u_h) - J(u) \\
    &= J(u_H) - J(u) + J(u_h) - J(u_H) \\
    &= E_H + [J(u_h) - J(u_H)] \\
    &= E_H + \langle \tilde{J}'(u_h,u_H), u_h - u_H \rangle,
\end{split}
\end{equation}
using the Taylor representation above.
Since $J$ satisfies the sufficient descent condition, we have
\begin{equation}
\begin{split}
E_h &=     E_H + \langle \tilde{J}'(u_h,u_H), u_h - u_H \rangle \\
    &\leqs E_H - \alpha E_H \\
    &= (1-\alpha)E_H.
\end{split}
\end{equation}
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Adaptive algorithms (Banach Presheaf Version)} 

\mnote{
KEY PLAY:  We now show how to construct such a sequence in an adaptive
setting, i.e., a sequence which converges and such that the residual
converges weakly zero.
}
According to the general framework developed in Section~\ref{sec:weak_framework}, the remaining question is how to construct the subspaces $X_k$ and $Y_k,$ as well as to find the approximate solution $u_k\in X_k$ of $u.$
For this purpose, we formulate a generalized adaptive finite element algorithm for solving the equation \eqref{eqn:model}, and make some basic assumptions on the algorithm.

Since the algorithm to be analyzed is of a finite element type, we need to have as the spaces $X$ and $Y$ function spaces defined over a domain in $\R^n$, or over a manifold.
The manifold setting is more general because a domain is trivially a manifold; however, in order to avoid the differential geometric language
we consider here the even more general setting of measure spaces, which
allows for a simple and transparent discussion of the core ideas.


We are interested in understanding the structure and convergence behavior of generalized adaptive finite element algorithms which have the form:
\begin{enumerate}
    \item[(1)] $u_k:=$ \textsf{SOLVE}($X(P_k), Y(P_k)$).
    \item[(2)] $\{\eta_k(\tau)\}_{\tau\in P_k}:=$ \textsf{ESTIMATE}($u_k, P_k$).
    \item[(3)] $\cM_k:=$\textsf{ MARK}($\{\eta_k(\tau)\}_{\tau\in P_k}, P_k$).
    \item[(4)] $P_{k+1} :=$\textsf{REFINE}($P_k, \cM_k$).
\end{enumerate}
Here, $\eta_k(\tau)$ is a localized error indicator that is used to drive enrichment of the approximation space, and will be defined more precisely below.
In practice, a stopping criteria is placed in Step (2) to terminate the loop, based on achieving a desired approximation quality.

\mnote{
More work needed here.
-mjh
}

Let $(\Omega,\Sigma,\mu)$ be a measure space, where $\Omega$ is a set, $\Sigma$ is a $\sigma$-algebra, and $\mu:\Sigma\to[0,\infty]$ is a measure.
Recall that a {\em $\sigma$-algebra} $\Sigma\subseteq2^{\Omega}$ over $\Omega$ is a collection of subsets of $\Omega$ which contains $\Omega$, and is closed under the complement in $\Omega$ and countable union operations.
Then a measure $\mu:\Sigma\to[0,\infty]$ is a function with $\mu(\emptyset)=0$ and additive under disjoint countable unions.

Let $\Sigma^e$ be a set of nonzero measure subsets that generates $\Sigma$.
We call $\Sigma^e$ the set of {\em elements}.
Fix a constant $C_P>0$.
Then, we say that $P\subset\Sigma^e$ is a {\em partition} of $\Omega$ if it is a uniformly locally finite covering of $\Omega$,
i.e., if $\cup_{\tau\in P}\tau=\Omega$, and $\#\{\tau\in P : x\in\tau\}\leqs C_P$ for any $x\in\Omega$.
We will denote the set of all partitions of $\Omega$ by $\cP$.
Note that $\cP$ depends on the choice of the constant $C_P$.

We assume that a {\em refinement rule} is given for any element,
namely, there is map 
$$\mathrm{refs}:\Sigma^e\to2^{\Sigma^e}$$ 
such that
for any $\tau\in\Sigma^e$, and for $S=\mathrm{refs}(\tau)$ 
we have $\tau\subseteq\cup_{\sigma\in S}\sigma$ and $\#S\lesssim 1.$ Moreover, there exists some constant $\alpha<1$, such that $\mu(\sigma)\leqs\alpha\mu(\tau)$ for $\sigma\in S.$
We say that $P'\in\cP$ is a {\em refinement} of $P\in\cP$ if 
for any $\sigma\in P'$, there is $\tau\in P$ such that $\sigma\in\{\tau\}\cup\mathrm{refs}(\tau)\cup\mathrm{refs}(\mathrm{refs}(\tau))\cup\ldots$,
where the notation is self-explanatory: $\mathrm{refs}(\mathrm{refs}(\tau))=\cup_{\nu\in\mathrm{refs}(\tau)}\mathrm{refs}(\nu)$, and so on.
Denoting the set of all refinements of $P$ by $\mathrm{refs}(P)$ this relation can be written as $P'\in\mathrm{refs}(P)$.

Given a partition $P$, the idea now is to construct certain subspaces $X_P\subset X$ and $Y_P\subset Y$ and discretize the equation 
\eqref{eqn:model} as in \eqref{eqn:nonlinear_galerkin}.
In general, we will not be able to do this for any partition $P\in\cP$;
thus we will restrict our attention to a subclass $\cP^a\subseteq\cP$,
which will be called the set of {\em admissible partitions}.
Namely, we assume that for every admissible partition $P\in\cP^a$
there exist Banach spaces $X_P\subset X$ and $Y_P\subset Y$ such that
\begin{equation}
\label{eqn:conforming-presheaf}
P'\in\mathrm{refs}(P)\cap\cP^a \mbox{ implies } X_{P}\subset X_{P'} \mbox{ and }Y_{P}\subset Y_{P'}.
\end{equation}


%\paragraph{\textsf{MARK} and \textsf{REFINE}}

Suppose that  an admissible partition $P\in\cP^a$ is given,
and that we computed $u_P\in X_P$ a solution of the equation \eqref{eqn:nonlinear_galerkin}.
One of the key step in the loop is to estimate the distribution of the error $\|u-u_P\|_X$ over the elements $\tau\in P$ by 
some means, and then refine the elements that are estimated to be sharing a large fraction of the error.
In what follows, the operation that selects the elements to be refined is analyzed via the map called ``$\mathrm{mrk}$'',
and the refinement procedure is analyzed via the map called ``$\mathrm{ref}$''.
After the refinement, we are supposed to get a new admissible partition and repeat the process 
until one is satisfied with the estimated error.

With $T\cP^a:=\cup_{P\in\cP^a}\{P\}\times2^P$,
we assume the existence of the following two maps
\begin{equation*}
\mathrm{mrk} : \cP^a \to 2^{\Sigma^e},
\qquad
\mathrm{ref} : T\cP^a \to \cP^a,
\end{equation*}
satisfying $\mathrm{mrk}(P)\subseteq P$ and $\mathrm{ref}(P,M)\supset\mathrm{refs}(\tau)$ for any $\tau\in M$.
In words, given  an admissible  partition $P$, $\mathrm{mrk}$ selects a subset $M\subseteq P$,
and given an admissible partition $P$ and a subset $M\subseteq P$, $\mathrm{ref}$ 
returns another admissible partition that contains (at least) refinements of the elements in $M$.
The convergence behavior of the algorithm depends crucially on the properties of $\mathrm{mrk}$.

On account of the above, the analysis of the adaptive algorithm can be reduced to the study
of the sequence $P_0,P_1,\ldots$ of admissible partitions, where $P_0\in\cP^a$ is the initial partition and 
\begin{equation}
\label{eqn:adaptive-presheaf}
P_{i+1}=\mathrm{ref}(P_i,\mathrm{mrk}(P_i)), \qquad i\in\N,
\end{equation}
and of $u_i\in X_i:=X_{P_i}$ ($i\in\N_0$), which is a solution to the discrete Petrov-Galerkin problem
\begin{equation*}
\langle F(u_i),  v\rangle =0.\qquad v\in Y_i:=Y_{P_i}.
\end{equation*}
The existence and uniqueness of $u_i$ are given by 
Theorems in Section~\ref{sec:weak_framework}.
We introduce some auxiliary concepts into the analysis.

\begin{definition}
\label{def:presheaf}
For $q>1$,
an {\em $\ell^q$-Banach presheaf} $Z$ over $\Omega$ is given by the following data
\begin{itemize}
\item[(i)] 
For each $U\in\Sigma$, a Banach space $Z(U)$;
\item[(ii)] 
For any $U,V\in\Sigma$ with $V\subseteq U$, a bounded linear projector $R_{U,V}:Z(U)\to Z(V)$;
\end{itemize}
satisfying
\begin{itemize}
\item[(a)] 
For any $U,V,W\in\Sigma$ with $W\subseteq V\subseteq U$, $R_{V,W}\circ R_{U,V} = R_{U,W}$;
\item[(b)] 
For any $U,V\in\Sigma$ with $V\subseteq U$,
$$
\|v\|_{Z(U)}\lesssim \|R_{U,V}v\|_{Z(V)} + \|R_{U,U\setminus V}v\|_{Z(U\setminus V)},
\qquad v\in Z(U);
$$
\item[(c)] 
For any partition $S$ of $U\in\Sigma$
$$
\|(\|R_{U,\tau}v\|_{Z(\tau)})_{\tau\in S}\|_{\ell^q} \lesssim \|v\|_{Z(U)},
\qquad v\in Z(U);
$$
\item[(d)] 
If $\{\tau_i\}\subset\Sigma$ is a sequence
with $\mu(\tau_i)\to0$ as $i\to\infty$, then for any $v\in Z$,
$\|R_{\Omega,\tau_i}v\|_{Z(\tau_i)}\to0$.
\end{itemize}
The projectors $R_{U,V}$ will be called the {\em restriction operators}, and if there is no risk of confusion, 
we will omit the domain $U$ in the notations, e.g., $R_V=R_{U,V}$.
\end{definition}

Without the local structure, a Banach presheaf $Z$ is simply the Banach space $Z(\Omega)$,
and in this sense we assume that the spaces $X$ and $Y$ are respectively $\ell^p$- and $\ell^q$-Banach presheaves over $\Omega$.

Next, we assume that the system $\{Y_P:P\in\cP^a\}$ is {\em locally dense} in $Y.$ Namely, for any $U\in\Sigma$ and any sequence $(P_i)_{i\in\N}$ of admissible partitions
satisfying 
$$\inf\{\mu(\tau):\tau\in P_i,\,\tau\ni x,\,i\in\N\}=0$$ for all $x\in U$,
the set $R_{U}\cup_iY_{P_i}$ is dense in $Y(U).$
In most conforming finite element spaces in Sobolev spaces, this is an immediate consequence of the usual interpolation error estimate, cf.~\cite{Ciarlet.P1978}.

%\paragraph{\textsf{ESTIMATE}}
\begin{assumption}\label{a:err-ind}
We assume that there exists a family of functions 
$\eta_P:P\to\R_+$ ($P\in\cP^a$), satisfying the following conditions.
\begin{itemize}
\item[(i)]
For any $S \subset P$ and $v\in Y$
\begin{equation}\label{e:est-up-bnd-presheaf}
\langle F(u_{P}), v\rangle 
\lesssim
\eta_{P}(S) \|R_{\Omega_S} v\|_{Y(\Omega_S)} 
+ \eta_{P}(P\setminus S)\|R_{\Omega_{P\setminus S}}v\|_{Y(\Omega_{P\setminus S})},
\end{equation}
where $\eta_P(S) = \| (\eta_P(\tau))_{\tau\in S}\|_{\ell^p}$
for any subset $S\subset P$,
and
$\Omega_{S}=\cup_{\{\sigma\in S\}}\sigma$ for $S\in\Sigma$.
\item[(ii)]
There exists a function $D\in L^p(\Omega)$ such that
\begin{equation}\label{e:est-stab-presheaf}
\eta_{P}(\tau) 
\lesssim
 \|R_{\tau}u_{P}\|_{X(\tau)} + \|D\|_{L^p(\tau)},
\qquad 
\tau \in P,
\end{equation}
\item[(iii)]
There exists a continuous function $\xi:\R_+\to\R_+$ with $\xi(0)=0$ such that
\begin{equation}\label{e:est-mark-presheaf}
\eta_{P}(\tau) 
\leqs
\xi\big(\max_{\sigma\in \cM}\eta_{P}(\sigma)\big),
\qquad 
\tau\in P\setminus \cM,\,
\cM=\mathrm{mrk}(P).
\end{equation}
\end{itemize}
\end{assumption}
\begin{remark}
We remark that the stability assumption (ii) is weaker than the local lower bound bound.
As we can see from the examples in Section~\ref{sec:examples}, one can obtain the stability estimate~\ref{e:est-stab-presheaf} from the local lower bound.
\end{remark}

The quantities $\eta_P(\tau)$ will be referred to as {\em local error indicators},
and $\eta_P(P)$ will be referred to as the {\em error estimator}.
This terminology may be justified by the fact that the choice $S=P$ in \eqref{e:est-up-bnd-presheaf} implies
\begin{equation}
\|u - u_{P}\|_X \lesssim \|F(u_{P})\|_{Y'} \lesssim \eta_{P}(P).
\end{equation}

\mnote{
Two paragraphs to add here:
(1) Show what the algorithm looks like in the simple case of 
    the domain $\Omega \subset \mathbb{R}^n$.
(2) Show what it looks like for a $n$-manifold.
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Differentiable Manifolds, Submanifolds, and Submersions}

Let $G : X \rightarrow Y$, where $X$ and $Y$ are Banach spaces.
Consider an implicitly defined {\em manifold} $\mathcal{M} \subseteq X$,
characterized as a the zero level-set of the mapping $G$:
\begin{equation}
   \label{eqn:constraint}
\mathcal{M} = \left\{ ~ u \in \mathcal{D}(G) \subseteq X
                     ~|~ G(u) = 0 \in \mathcal{R}(G) \subseteq Y ~\right\}.
\end{equation}
An {\em admissible curve} or {\em admissible path}
in $\mathcal{M}$ through $u \in \mathcal{M}$ is
a differentiable mapping
$\gamma(t) : (-t_0,t_0) \rightarrow \mathcal{M}$,
for some $t_0 > 0$, with $\gamma(0) = u$.
A vector $v \in X$ is called a {\em tangent vector} to $\mathcal{M}$
at $u$ if there exists an admissible path $\gamma(t)$ to $\mathcal{M}$
at $u$ such that $\gamma^{\prime}(0) = v$.
The set of tangent vectors at a point $u \in \mathcal{M}$
form a vector space $T_u \mathcal{M}$ known as the {\em tangent space}
of $\mathcal{M}$ at $u$:
\begin{equation}
T_u\mathcal{M} = \{~ v \in X ~|~ \dot{\gamma}(0) = v,
                  ~\text{with}~ \gamma(t) ~\text{an~admissible~path~in}~
                   \mathcal{M} ~\text{through}~ u ~\}.
\end{equation}
The {\em tangent bundle} $T\mathcal{M}$ of a manifold $\mathcal{M}$
is the union of the tangent spaces at all points $u \in \mathcal{M}$:
\begin{equation}
T\mathcal{M} = \bigcup_{u \in \mathcal{M}} T_u \mathcal{M}.
\end{equation}
A particular tangent space $T_u \mathcal{M}$ is called a {\em fiber} of
the tangent bundle $T\mathcal{M}$ at $u \in \mathcal{M}$.
The map $\pi_{\mathcal{M}}:T\mathcal{M}\rightarrow \mathcal{M}$ which maps tangent
vectors to their attachment points on $\mathcal{M}$ is called the
{\em natural projection} operator, and the inverse image $\pi_{\mathcal{M}}^{-1}$
of $\pi_{\mathcal{M}}$ assigns a fiber $T_u\mathcal{M}$
of the tangent bundle $T\mathcal{M}$ to each point $u \in \mathcal{M}$.
A {\em vector field} on $\mathcal{M}$ is a map $V : \mathcal{M} \rightarrow T\mathcal{M}$,
so that a vector $V(u) \in T_u\mathcal{M}$ is assigned to each $u \in \mathcal{M}$.
The vector space of bounded linear functionals on the tangent space
$T_u\mathcal{M}$ is the {\em cotangent space} $T_u^*\mathcal{M}$,
and the disjoint union of the cotangent spaces
is called the {\em cotangent bundle} $T^*\mathcal{M}$:
\begin{equation}
T^*\mathcal{M} = \bigcup_{u \in \mathcal{M}} T_u^* \mathcal{M}.
\end{equation}
Analogously, $T_u^*\mathcal{M}$ is called a fiber of the
cotangent bundle $T^*\mathcal{M}$ at $u \in \mathcal{M}$.

A property of nonlinear mappings that we will use repeatedly in these
notes in the case of implicitly defined manifolds is {\em submersion}.
A mapping $G : \mathcal{D}(G) \subseteq X \rightarrow Y$ is called
a {\em submersion} at $u$ if the following three conditions hold:
\begin{enumerateX}
\item $G(u)$ is $C^1$ in a ball around $u$.
\item $G^{\prime}(u) : X \rightarrow L(X,Y)$ is a surjective linear
      operator at $u$ (i.e., $\mathcal{R}(G^{\prime}) = Y$).
\item There exists a linear projection operator $P$
      which splits $X$ into $\mathcal{N}(G^{\prime}(u))$ and
      $\mathcal{N}^{\perp}(G^{\prime}(u))$.
\end{enumerateX}
Note that if $X = \mathbb{R}^n$ and $Y=\mathbb{R}^m$, then 2) is equivalent
the assumption that $G^{\prime}(u)$ has full rank, and then
3) follows from the fact that
$\mathcal{N}(G^{\prime}(u)) \perp \mathcal{R}(G^{\prime}(u)^T)$,
so that
$X=\mathbb{R}^n \equiv \mathcal{N}(G^{\prime}(u)) \oplus \mathcal{R}(G^{\prime T}(u))$.

If $G : X \rightarrow Y$ is a submersion at $u \in \mathcal{M}$,
a classical result due to Ljusternik
(cf.~Theorem 43.C in~\cite{Zeid91c}) gives a useful alternative
characterization of the tangent space $T_u\mathcal{M}$ which will make it
possible to develop a very general framework for Lagrange functionals
and multipliers in the next section:
\begin{equation}
   \label{eqn:ljust}
T_u\mathcal{M} \equiv \mathcal{N}(G^{\prime}(u))
            = \{~ v \in X ~|~ G^{\prime}(u)v = 0 \in Y ~\}.
\end{equation}
In other words, the tangent space is precisely the null
space of the derivative of the operator $G$ implicitly defining
the manifold $\mathcal{M}$.
Moreover, Ljusternik's result is also that there exists local structure
(an atlas of charts), giving $\mathcal{M}$ the mathematical structure
of a $C^1$ manifold (or {\em differentiable manifold}).
The differentiable manifold structure allows for the construction of
derivatives, differentials, and directional derivatives of various
types of functions having $\mathcal{M}$ is their domain, providing
an intrinsic differential calculus on $\mathcal{M}$ that does not
depend extrinsically on $X$ through the relationship $\mathcal{M} \subseteq X$.
The differentiable manifold structure provided by the constraint operator
may be exploited to solve constrained evolution problems using numerical
algorithms which never depart from $\mathcal{M}$ (cf.~\cite{HLW01}).


